StarHarness: Evolving Harnesses with Stratified Search for Enterprise Environments

We present StarHarness, a framework for evolving environment-specific agent harnesses while keeping model weights fixed. The evolved harness can include prompt and task framing, tool interfaces, skills, MCP-backed providers, subagent structure, and agent-loop configuration. StarHarness constructs a compact evolution pool by stratifying tasks according to baseline failure behavior, separates proposer-visible search tasks from proposer-hidden selection tasks, and reserves held-out tasks for evaluating generalization. Across ITBench SRE, EnterpriseOps-Gym ITSM, and AutomationBench Finance, harness evolution improves full-benchmark performance by 20-35 percentage points over the default harness after 4-12 accepted changes per environment. These gains persist on tasks excluded from evolution and transfer without re-evolution across GPT and Qwen model families. Trace analysis links the improvements to interface repairs, environment conventions, and operational knowledge that compresses search, with fewer false-positive diagnoses and shorter trajectories in several settings. StarHarness therefore offers a practical way to reduce persistent model-environment mismatch in tool-rich enterprise tasks.

==> ServiceNow/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ServiceNow/sections/abstract.tex <==
\begin{abstract}
    Reliable LLM agents for enterprise software must act in interconnected, stateful, policy-governed environments shaped by organizational history. Existing benchmarks often create difficulty through authored prompts and hand-built database states, obscuring a core property of real deployments: the same request may be easy, hard, or infeasible depending on context. We introduce \ours, a benchmark where difficulty emerges from the environment rather than the task description. The benchmark uses a two-phase pipeline: a simulation evolves policy-constrained enterprise states across HR, ITSM, and CSM, and verified workflows generate tasks with oracle trajectories, database-diff verifiers, and infeasible variants. Executable policies and generators enable mechanical consistency checks and outcome-based verification without LLM judges. The benchmark evaluates workflow following, novel-scenario reasoning, cross-domain orchestration, and infeasibility detection.  Experiments with frontier models show that [key result placeholder]. Our analysis further suggests that [key finding placeholder]. These results position evolved enterprise environments as scalable infrastructure for benchmarking, safe agent evaluation, and reinforcement learning from verifiable software states.
\end{abstract}

==> ServiceNow/sections/conclusion.tex <==
\section{Conclusion}

We introduced \ours{}, a benchmark for evaluating enterprise agents in evolved, causally rich software worlds. Rather than placing difficulty in the prompt, \ours{} makes it emerge from accumulated state: prior actions, linked records, policies, cross-domain dependencies, and infeasible conditions. Its executable environment representation generates tasks, oracle trajectories, and exact verifiers from valid state transitions, enabling evaluation of workflow execution, discovery, orchestration, and safe refusal.

More broadly, \ours{} points toward reinforcement learning environments for enterprise agents. With policy-checked actions, grounded state transitions, exact success signals, and snapshots of increasing causal depth, it provides a foundation for training agents that learn when to act, how to recover, how to coordinate across systems, and when to refuse. This moves enterprise-agent evaluation from static, prompt-authored tasks toward living environments for verifiable learning under realistic operational complexity.

==> ServiceNow/sections/discussion.tex <==
\section{Discussion}

==> ServiceNow/sections/introduction.tex <==
\section{Introduction}

Large language models are shifting from passive assistants that answer questions toward agents that take consequential actions on behalf of users~\citep{xu2026theagentcompany,yao2025taubench}. Increasingly, these agents do not act alone: they operate alongside people, requesting approvals, escalating decisions, and coordinating with other actors to get work done. Enterprise software is where this shift matters most. It is where organizations run their day-to-day operations, where actions carry real consequences, and where even modest gains in agent reliability translate into large practical impact. In these settings, what counts as "the task" is not fully contained in the user's request. It is shaped by the surrounding operational world in which the instruction is embedded. That world is not a static backdrop but an executable structure, the schema, policies, tools with their preconditions, and supporting actors that admits many possible trajectories, of which any given request is only one. A request such as closing an incident, activating a contract, or processing an offboarding case may require the agent to inspect linked records, identify which policy applies, determine whether it has authority to proceed, and proactively ask the right supporting actor for missing approval or information. The instruction may be short, but successful execution depends on understanding the environment around it.

Existing agent benchmarks have driven progress on tool use, web interaction, and workplace automation~\citep{qin2024toolllm,xu2026theagentcompany,malay2026enterpriseopsgym,shepard2026automationbench}. Yet many make tasks hard by placing the difficulty in the prompt rather than the world. Instructions are lengthened, goals are composed, distractors are introduced, or relevant procedure is hand-encoded in a bespoke setup. These designs are valuable probes of planning and tool selection, but they only partially reflect enterprise operations. The real difficulty for enterprise AI is discovering what the current world permits and what must happen before taking action. While a user typically issues an ordinary request, the surrounding system state introduces immediate friction: the agent must navigate situations where a policy demands an approval, an entitlement has gone stale, or an incident is linked to a prior problem. Progress can also stall if a change freeze blocks the next step or if another actor has already altered the record. Recent work echoes this point, showing that frontier agents suffer from \textit{dynamics blindness}---they fail to anticipate the hidden, cascading side effects of their actions and require grounded world modeling to stay reliable in opaque enterprise systems~\citep{gupta2026world, nair2026enterprise}.


\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/teaser-v7.png}
    \caption{
    \textbf{Difficulty lives in the environment, not the prompt.}
    \ours{} generates diverse, policy-governed enterprise worlds in which the same request can require fundamentally different agent behavior. Depending on the surrounding records, dependencies, actors, and constraints, an offboarding request may be completed directly, require investigation and multi-party coordination, or become impermissible and call for a safe refusal. The examples shown are illustrative: even with the request held fixed, changes in the underlying world state can alter what information is relevant, which actions are valid, and whether the task is feasible at all.
}
   
    \label{fig:teaser}
\end{figure*}





We introduce \ours{}, a framework for generating and studying enterprise-agent tasks inside executable enterprise worlds. Each world (Figure~\ref{fig:teaser}) is built from five components: an ontology and mutable data that specify the structure and current state of the environment, policies that constrain how that state may evolve, tools that expose the actions available to agents, and process knowledge that encodes how enterprise work is carried out. Rather than authoring each task by hand, \ours{} builds worlds in which tasks \emph{arise} from valid state transitions. The leverage comes from moving the authored surface upstream: we do not write tasks, we write the \emph{processes} that produce them---parameterized workflows, the policies that govern them, and the tools that execute them---so a single authored process yields many tasks, each bound to a different slice of the world and each carrying its own oracle trajectory and verifier by construction. This lets us isolate the properties that make enterprise work hard such as policy-grounded reasoning, proactive coordination with supporting actors, safe refusal, cross-domain side effects, and sensitivity to accumulated history, and vary them in a controlled way.



Our framework is built around a deliberate \emph{information asymmetry between world construction and agent evaluation}. When the world is constructed, a policy oracle checks every action before it can modify the database, so the resulting states and trajectories are valid by design. At evaluation time this oracle is withheld: organizational policies are no longer enforced by the tools, and the agent must instead discover the relevant rules from ordinary workspace knowledge, wiki articles and SOPs---then decide whether it can act, needs approval from another actor, or should abstain rather than corrupt the environment---a clean refusal that current agents often fail to make, complying under pressure and leaving partial or state-corrupting side effects instead~\citep{yao2025taubench,barres2025tau2}. Because difficulty now lives in the state rather than the prompt, the same short request can range from routine to impossible depending on the world it lands in, and we can raise difficulty systematically by evolving more history, adding cross-domain dependencies, or changing which policies are visible.

We instantiate this framework in enterprise operations spanning IT service management (ITSM), customer service management (CSM), and human resources (HR). The environment contains relational enterprise state, domain-specific tools, organizational policies, executable workflows, SOPs, wiki knowledge, and supporting personas with roles and responsibilities. We fix an enterprise world once, then bind each workflow onto it by provisioning the local slice of state its preconditions require; simulation then evolves the initial seed through policy-valid activity, producing snapshots with linked incidents, approvals, entitlements, employee records, customer cases, contracts, and cross-domain dependencies. Tasks are derived from these evolved snapshots and packaged with the information available to an agent at test time, together with oracle trajectories and verifier specifications retained for evaluation. Using this framework, we analyze enterprise-agent performance across workflow execution, policy reasoning, coordination, and
safe refusal, and we study how test-time scaffolding (harness and memory) and fine-tuning affect these capabilities.\todo{are we really doing this though?}

Our contributions are as follows:

\begin{itemize}
    \item We introduce \ours{}, a framework for constructing executable enterprise worlds in which agent tasks arise from accumulated state, policy constraints and interactions with supporting actors rather than from manually authored prompt complexity.


    \item We propose a two-phase construction pipeline that first procedurally generates enterprise processes---workflows, policies, and tools---and binds them onto a fixed world, then simulates policy-valid workflow activity to derive tasks with oracle trajectories and verifier specifications. Because the authored unit is the process rather than the task, one process scales to many verified tasks, enabling controlled evaluation of workflow execution, policy-grounded reasoning, coordination with supporting personas, infeasibility detection, and safe refusal.

    \item We evaluate a range of enterprise agents across these capabilities and study interventions for improving them, showing how test-time scaffolding and fine-tuning affect policy reasoning, coordination, side-effect control, and safe refusal.
\end{itemize}

==> ServiceNow/sections/limitations.tex <==
\section*{Limitations}

\ours{} represents an important step toward dynamic environments for agent training and evaluation, but the current simulation engine still abstracts away several forms of enterprise-world evolution. We define an enterprise environment through five core elements: an ontology, a mutable database, a set of policies, a tool surface, and knowledge sources. In the present implementation, however, only the database state evolves over time. This captures an important class of enterprise dynamics, since most operational tasks involve reading from and writing to persistent records, but it does not fully reflect the broader evolution observed in real organizations. In practice, schemas change as new data models are introduced, policies are revised as organizational rules evolve, tools are added or deprecated, and knowledge bases are continuously updated.

A natural direction for future work is therefore to extend the simulator beyond mutable database state and toward environments in which agents or external processes can also modify policies, knowledge sources, and tools through interaction. This would enable richer forms of long-horizon adaptation, where agents must not only operate within an existing enterprise world but also help reshape the world itself. Such extensions would make it possible to study settings where process knowledge becomes stale, policy changes invalidate previously successful strategies, or new tools alter the space of feasible actions. \textcolor{red}{Add limitations in real prod systems: they are siloed and offer a partially visible agent action surface}

==> ServiceNow/sections/methods.tex <==
\section{Methods}

\ours{} is a framework for constructing enterprise-agent benchmarks from executable software worlds. Its central premise is that task difficulty depends not only on the user request, but also on the surrounding environment: its current state, organizational policies, available information, and other actors. To generate such tasks reliably, \ours{} exploits an \emph{information asymmetry between construction and evaluation}. During construction, workflows, policies, and actor behavior are available as structured, executable artifacts; during evaluation, they are projected into the records, documentation, tools, and interactions available to the agent. This privileged construction view lets us generate tasks of varying complexity while ensuring that feasible tasks have a valid solution and that all information needed to recover it remains accessible in the agent-facing world.

\subsection{Executable Enterprise Worlds}

We represent an enterprise environment as a tuple
\[
E = (O, D, P, T, K),
\]
where $O$ is the ontology, $D$ is the mutable database state, $P$ is the set of policies governing valid transitions, $T$ is the tool surface, and $K$ is process knowledge. 

The ontology defines the relational schema of the world, including tables, fields, foreign-key constraints, closed enum sets, and domain-specific entity types. The database contains the records that instantiate this world at a given point in time. Supporting actors, their roles, and their relationships to other entities are also represented in this state.

Policies define which state transitions are valid. We distinguish two kinds of policy. \emph{Platform invariants} capture constraints that the software must always enforce, such as referential integrity, access control, and valid state transitions. \emph{Organizational policies} capture tenant-specific rules, such as separation of duties, approval chains, escalation requirements, and compliance procedures. For example, the platform may prevent a new incident from moving directly to a closed state, while an organization's policy may additionally require a senior executive to be informed before a security-related incident is closed. This distinction is important at evaluation time: platform invariants remain enforced, while the enforcement of organizational policies can be moved from the tool layer to the agent.

Tools are the only mechanism through which an agent can change $D$. Process knowledge $K$ includes executable workflows, policy definitions, and supporting-actor rules, as well as the SOPs and wiki articles derived from them. Because these components share a common formal representation, \ours{} can mechanically check that workflows invoke valid tools, tools reference valid schema fields, and executed transitions satisfy the applicable constraints.

\subsection{Information Asymmetry}

Benchmark construction and evaluation expose different views of the same enterprise process. During construction, \ours{} has access to an executable workflow, machine-checkable policies, selected workflow branches, and the expected behavior of supporting actors. During evaluation, this structure is projected into the interface of an enterprise agent.

The asymmetry affects three aspects of the task. First, the constructor observes and executes a reference trajectory, whereas the evaluated agent must infer an appropriate trajectory from the request and current state. Second, organizational policies can actively gate writes during construction but be surfaced only through documentation during evaluation. Third, structured workflow conditions and actor responses become distributed across SOPs, wiki articles, database records, tool outputs, and interactive actors.

We call this conversion an \emph{agent-facing projection}. The projection controls where relevant information appears and what the agent must do to obtain it, but it does not remove facts required for success. Every consequential decision on a feasible reference trajectory must be supported by an accessible source, such as the task instruction, a database record, a document, a prior tool result, or a supporting actor. For infeasible tasks, the blocking condition must likewise be discoverable. This \emph{information-completeness} requirement ensures that difficulty arises from discovery, reasoning, coordination, and execution rather than from missing benchmark context.

\subsection{World and Task Synthesis}

We formulate benchmark construction as valid trajectory sampling. Given an executable workflow, \ours{} selects a path, constructs a world in which its conditions hold, executes the path, and compiles the resulting trace into an agent-facing task and verifier. This process consists of three stages: \emph{Arrange}, \emph{Act}, and \emph{Assert}.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/task-synthesis-v4.png}
    \caption{\textbf{World and task synthesis from executable enterprise environments.}
Starting from a seed world defined by its ontology, database state, policies, tools, and process knowledge, \ours{} constructs benchmark tasks through three connected stages. \emph{Arrange} selects a workflow path and realizes its preconditions in the world; \emph{Act} executes the path through policy-gated tools and supporting actors, producing a valid trajectory; and \emph{Assert} projects this execution into agent-facing artifacts and verifies both execution validity and information completeness. A difficulty control plane varies world state, policy responsibility, information placement, coordination, and feasibility.}
    \label{fig:task_synthesis}
\end{figure}

\subsubsection{Arrange}

The Arrange stage selects a path through an executable workflow and provisions the entities and relationships required to realize it. Path conditions are translated into requirements on enterprise records, such as the employee, manager, group, incident, approval, entitlement, or customer that must exist for the workflow to take the selected branch.

The constructor first attempts to bind these requirements to entities already present in the seed world. When suitable entities do not exist, it creates or modifies records through the same policy-gated tool interface used during execution. Arrange may also introduce historical records and cross-domain dependencies needed to produce a desired level of state complexity. Its output is an initial state $D_0$ in which the selected workflow path is both reachable and internally consistent.

\subsubsection{Act: Execute Valid Work and Compile a Task}

In the Act stage, we execute the selected workflow on the bound entities. Every state-changing operation passes through policy-gated construction tools. A write that violates an applicable constraint is rejected, forcing construction to follow a compliant branch.

When a step depends on another party(such as a \textit{manager}, \textit{vice president}, \textit{customer}, or \textit{another department}), a supporting-actor controller supplies the response associated with the selected path. The response and its justification are recorded as actor metadata. At evaluation time, this metadata becomes a behavior rule for an interactive actor rather than information given directly to the agent.

A successful execution produces a golden trajectory
\[
\tau^*: D_0 \rightarrow D_1,
\]
containing the tool calls, parameters, observations, writes, policies, and actor interactions involved in completing the task. From this trace, \ours{} derives the expected database changes, side-effect constraints, supporting-actor rules, and agent-facing process documentation. The user instruction is generated from the completed work, producing a concise request grounded in a demonstrated, policy-compliant transition.

To construct infeasible variants, the Arrange stage instead provisions a world in which a necessary condition cannot be satisfied safely. Examples include an unavailable approval, a circular dependency, a missing required record, or an active change freeze. The Act stage then establishes that the correct outcome is to stop or refuse without making harmful partial changes.

\subsubsection{Assert}

The Assert stage validates both the execution and the agent-facing projection. Executable checks confirm that the golden tool calls are valid, the expected terminal state $D_1$ is reached, required changes appear in the database diff, unintended side effects are absent, and applicable platform and organizational constraints hold. These checks establish that the task and its verifier are consistent with a valid execution.

Execution validity alone does not guarantee that an evaluated agent could justify the same actions from its available context. We therefore perform an LLM-based provenance audit over the golden trajectory. For each consequential tool call and parameter, the judge checks whether the decision is supported by the task instruction, database observations, process documentation, prior tool results, or supporting-actor interactions. The rubric flags hidden construction assumptions, unexplained identifiers, missing policy conditions, unjustified actor choices, and blockers that are not discoverable from the agent-facing world.

Samples that fail this information-completeness test are rejected. We additionally compare the golden trajectory with the behavior of a strong test-time agent to identify cases where apparent agent failures instead reveal ambiguous or poorly surfaced evidence. Accepted samples therefore have both executable evidence of a correct outcome and semantic evidence that the outcome is recoverable from the projected environment.

\subsection{Difficulty Control Plane}

The privileged construction view exposes a set of controls for varying task difficulty without relying on increasingly elaborate user instructions. We vary five main dimensions:

\begin{itemize}
    \item \textbf{State and process:} workflow branch depth, accumulated history, linked-record reasoning, edge cases, and cross-domain dependencies;
    \item \textbf{Policy responsibility:} which organizational constraints are tool-enforced and which must be identified and followed by the agent;
    \item \textbf{Information placement:} whether relevant procedures and facts are directly supplied, retrieved from documentation, distributed across sources, or combined with the current state;
    \item \textbf{Coordination:} which supporting actors hold required information or authority, and whether they approve, reject, or request additional evidence;
    \item \textbf{Assistance and feasibility:} whether required clarification is provided, must be requested, or cannot be obtained because of a genuine blocker.
\end{itemize}

These controls produce matched task families in which similar requests and workflows are embedded in different worlds. For example, ``process this offboarding'' may require a short linear execution, investigation across linked records, policy lookup and manager approval, cross-domain cleanup, or a justified refusal (see Figure \ref{fig:teaser} for an example). Difficulty therefore reflects what the agent must discover and coordinate in the environment rather than the complexity of the wording itself.

The controls need not induce a strictly monotonic increase in empirical difficulty, since their effects may interact. We therefore measure realized difficulty through agent evaluation and use rejection sampling to retain tasks with the desired range of behaviors.

\subsection{Evaluation Protocol}

Each task contains a natural-language instruction, an initial environment snapshot, an agent-facing workspace, and an outcome verifier derived from the oracle transition. A feasible task succeeds when the final state contains the required changes, preserves the relevant invariants, and avoids unintended side effects. For an infeasible task, success requires identifying the blocker and stopping or refusing without corrupting the environment.

We evaluate agents in four complementary settings. In \emph{Known Workflow}, the relevant SOP is provided and the agent must execute it correctly under the current state and policies. In \emph{Novel Scenario}, the agent must inspect the environment and retrieve the appropriate process documentation before acting. \emph{Cross-Domain Orchestration} introduces dependencies across enterprise systems and supporting actors whose information or approval is required. \emph{Infeasibility Detection} tests whether the agent can recognize that a request cannot be completed safely and avoid harmful partial execution.

Together, these settings evaluate whether agents can do more than follow a prescribed procedure: they must locate relevant context, interpret organizational policies, coordinate with other actors, manage side effects across systems, and recognize when no valid action is available.


==> ServiceNow/sections/methods_old.tex <==
\section{Methods}

\ours{} is a framework for constructing enterprise-agent benchmarks from executable software worlds. Its starting point is that an enterprise task is not fully specified by the user's request. Whether an agent can safely complete a request also depends on the current database state, the organization's policies and procedures, and the information or approval held by other actors. A useful benchmark should therefore test whether an agent can discover and act on this surrounding context, without making success depend on facts that are absent from the environment.

To construct such benchmarks, \ours{} creates a deliberate \textit{information asymmetry between construction and evaluation}. During construction, the framework has a privileged view in which workflows are executable, organizational policies are machine-checkable, and the behavior of supporting actors is known. At evaluation time, this structure is projected into the interface available to an enterprise agent: workflows and policies become SOPs and wiki documents, relevant facts are distributed across records, and information or approval must be obtained from the appropriate actors. The privileged construction artifacts also provide a control plane for varying process branches, accumulated state, policy responsibility, information placement, coordination burden, and feasibility. The same short request can therefore require a direct execution, substantial investigation and coordination, or a safe refusal.

This construction provides two complementary forms of validation. Policy-gated execution demonstrates that feasible work can be completed and produces an oracle trajectory, database diff, and outcome verifier. An LLM-based provenance rubric then checks the semantic requirement that each oracle action and parameter is justified by evidence available in the agent-facing environment. Together, these checks help ensure that difficulty comes from planning, discovery, and execution rather than from missing benchmark context.

\subsection{Executable Enterprise Worlds}

We represent an enterprise environment as a tuple
\[
E = (O, D, P, T, K),
\]
where $O$ is the ontology, $D$ is the mutable database state, $P$ is the set of policies governing valid transitions, $T$ is the tool surface, and $K$ is process knowledge. The ontology defines the relational schema of the world, including tables, fields, foreign-key constraints, closed enum sets, and domain-specific entity types. The database contains the records that instantiate this world at a given point in time. Supporting actors, their roles, and their relationships to other entities are also represented in this state.

We distinguish two kinds of policy. \emph{Platform invariants} capture constraints that the software must always enforce, such as referential integrity, access control, and valid state transitions. \emph{Organizational policies} capture tenant-specific rules, such as separation of duties, approval chains, escalation requirements, and compliance procedures. For example, the platform may prevent a new incident from moving directly to a closed state, while an organization's policy may additionally require a vice president to be informed before a security-related incident is closed. This distinction is important at evaluation time: platform invariants remain enforced, while the enforcement of organizational policies can be moved from the tool layer to the agent.

Tools are the only mechanism through which an agent changes $D$. During construction, every write through $T$ is checked against the applicable policies in $P$. Process knowledge $K$ consists of executable workflows, policy definitions, and rules for supporting actors, together with the SOP and wiki documents derived from these artifacts for the agent-facing workspace. This representation makes structural and execution consistency mechanical: tools must reference real schema fields, workflows must call valid tools with valid arguments, and completed trajectories must satisfy the policy suite. These checks establish that a trajectory is executable and policy-compliant, but not that every choice in it is justified by the information shown to the evaluated agent. Establishing that stronger form of sample validity requires the provenance validation described in Section~\ref{sec:assert-validation}.

\subsection{Privileged Construction and Agent-Facing Projection}

Information asymmetry has previously been used to make task synthesis easier than task solving. For example, \citet{xie2026agentsynth} constructs a solution forward, one tractable step at a time, and asks the evaluated agent to recover the resulting composite trajectory. We use the same trajectory asymmetry, and extend the privileged view to the policy-governed and multi-actor structure of enterprise work.

The construction and evaluation views differ along three main axes:

\begin{itemize}
    \item \textbf{Trajectory.} During construction, the oracle executes a selected branch of an executable workflow and thereby demonstrates a reference solution. During evaluation, the agent receives the user request and process documentation, and must determine the appropriate trajectory from the state it observes.

    \item \textbf{Enforcement.} During construction, organizational policies actively gate tool calls, so a violating write fails loudly and can be corrected. During evaluation, platform constraints remain enforced, but selected organizational policies are no longer enforced by the tools. The agent must identify and follow these rules before committing a write.

    \item \textbf{Specification and interaction.} During construction, policies, workflow branches, and required responses from supporting actors are available as structured artifacts. During evaluation, the same information is expressed through SOPs, wiki articles, enterprise records, and interactive actors. The agent must locate the relevant source, interpret it, and decide whom to contact for information or authorization.
\end{itemize}

We refer to the conversion from the privileged construction view to the agent-facing environment as a \emph{projection}. A projection does not arbitrarily hide facts needed for success. Instead, it determines where those facts appear and what work the agent must perform to obtain them. For every decision on a feasible reference trajectory, we require a corresponding agent-accessible source: the task instruction, a database record, an SOP or policy article, a tool result, or a supporting actor. For an infeasible task, the environment must likewise contain accessible evidence of the blocker. This \emph{information-completeness} requirement separates difficulty due to planning and discovery from difficulty caused by an underspecified benchmark. Because this is a semantic property rather than a database invariant, we validate it with an LLM-based provenance rubric.

\subsection{World and Task Synthesis}

We cast benchmark construction as valid trajectory sampling. Given an executable workflow, we select a path through it, provision a world in which its preconditions hold, execute the workflow through policy-gated tools, and compile the resulting trace into an agent-facing task and verifier. We organize this process into three stages: \emph{Arrange}, \emph{Act}, and \emph{Assert}.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/task-synthesis-v3.png}
    \caption{\textbf{World and task synthesis from executable enterprise environments.}
Starting from a seed world defined by its ontology, database state, policies, tools, and process knowledge, \ours{} constructs benchmark tasks through three connected stages. \emph{Arrange} selects a workflow path and realizes its preconditions in the world; \emph{Act} executes the path through policy-gated tools and supporting actors, producing a valid trajectory; and \emph{Assert} projects this execution into agent-facing artifacts and verifies both execution validity and information completeness. A difficulty control plane varies world complexity, policy burden, knowledge access, coordination requirements, and task feasibility, yielding tasks that range from simple to interdependent or policy-blocked.}
    \label{fig:task_synthesis}
\end{figure}

\subsubsection{Act: Execute Valid Work and Compile a Task}

In the Act stage, we execute the selected workflow on the bound entities. Every state-changing operation passes through the policy-gated construction tools. If an action violates an applicable policy, it is rejected and the construction process must follow a compliant branch. For steps that depend on another party (such as a \textit{manager}, \textit{vice president}, \textit{customer}, or \textit{another department}) a healer tracks the required interaction and supplies the response specified by the selected path. These responses and their justifications are recorded as actor metadata; at evaluation time, they become behavior rules for interactive NPCs rather than information given directly to the agent.

A successful execution produces a golden trajectory $\tau^*$ from initial state $D_0$ to final state $D_1$. The trace records the tools called, parameters supplied, records read and written, policies applied, supporting actors involved, and context available at each decision. We then derive the benchmark artifacts from this trace. The difference between $D_0$ and $D_1$ supplies the expected state change and side-effect constraints. The workflow and policy artifacts are translated into SOP and wiki documents. Finally, a short user request is generated from the work that was performed. Generating the instruction after the execution keeps the request natural while grounding it in demonstrated, policy-compliant work.

For infeasible variants, we provision a state in which a required condition cannot be satisfied safely: for example, an approval is unavailable, a dependency is circular, a required record has been deleted, or a change freeze blocks the operation. The expected outcome is then a justified refusal or stop with no harmful partial writes. As with feasible tasks, the blocker must be discoverable through the agent-facing environment.

\subsection{Difficulty Control Plane}

The privileged construction artifacts expose a control plane over both task generation and evaluation. Rather than equating difficulty with trajectory length, we vary the sources of work an agent must perform:

\begin{itemize}
    \item \textbf{State and process.} We select different concolic paths and bind them against worlds with different amounts of accumulated history. This varies branch depth, linked-record reasoning, edge cases, and cross-domain dependencies.

    \item \textbf{Policy responsibility.} We choose which organizational policies remain enforced by tools and which become the agent's responsibility. At one extreme, tools prevent most invalid actions; at the other, the agent must read the relevant policies and avoid policy-violating writes on its own.

    \item \textbf{Information placement.} We vary whether the relevant procedure is supplied directly, available through retrieval, distributed across multiple articles, or must be combined with facts in the current state. The required information remains available, but the discovery and interpretation burden changes.

    \item \textbf{Coordination.} We vary which supporting actors hold required information or authority, whether they must be contacted proactively, and whether they approve, reject, or request additional evidence according to their rulebooks.

    \item \textbf{User assistance and feasibility.} We can provide additional clarification, withhold it until requested, or instantiate a genuine blocker. This moves a request between directly feasible, conditionally feasible, and infeasible settings while preserving an accessible basis for the correct decision.
\end{itemize}

These controls let us construct matched task families in which the user request and underlying workflow remain similar while the surrounding world changes. A request such as ``process this offboarding'' may therefore require a short linear execution, a policy lookup and manager approval, cross-domain cleanup, or a safe refusal. Difficulty comes from what the agent must discover and coordinate in the environment, not from making the request itself convoluted. Because different controls may interact, we do not assume that any single knob produces a perfectly monotonic increase in empirical difficulty; we measure difficulty through agent evaluation and use rejection sampling to retain the desired range of behaviors.

\subsection{Assert: Executable Checks and LLM-Based Validation}
\label{sec:assert-validation}

The\todo{should have all 3 stages (arrange, act, assert) within the same subsection} Assert stage combines checks that can be executed directly with semantic validation by an LLM judge. We first replay the golden trajectory\todo{do we even need to do this?} from $D_0$, verify that every tool call is valid, confirm that the expected terminal state is reached, and inspect the database diff for required changes and unintended side effects. We also check that platform invariants and applicable organizational policies hold. These checks establish that the sampled work is executable and policy-compliant, and that its verifier is consistent with the replayed outcome. They do not establish that an evaluated agent could have justified the same actions from its available context.

That remaining question, i.e. \emph{provenance}, is central to sample validity. An LLM judge reviews the golden trajectory step by step~\citep{zheng2023judging} together with the agent-facing task, SOP and wiki collection, database observations, prior tool results, and supporting-actor interactions. For every consequential tool call and parameter choice, the judge determines whether the choice is grounded in one or more of these sources. The rubric flags hidden construction-time assumptions, unexplained identifiers or values, missing policy antecedents, unjustified actor selection, and infeasibility claims whose blocker is not discoverable. We reject a sample when a required step cannot be grounded in information available to the agent. This provenance audit is how we operationalize information completeness; it is a required validation stage, not merely a measure of writing quality.

We apply the rubric in two complementary modes. First, we inspect the golden trajectory on its own for provenance, coherence, naturalness, and accidental hints. Second, we contrast the golden trajectory with a trajectory produced by a strong test-time agent. In our current implementation, we use Sonnet-5\todo{cite} with medium reasoning in a ReAct\todo{cite} orchestrator and provide it with the oracle SOP-KB. When this agent fails, the judge assesses whether the failure reflects an agent mistake or missing, ambiguous, or poorly surfaced evidence in the sample. We also score long-horizon interestingness and use rejection sampling to retain the desired difficulty profile.

Sample validity therefore rests on both executable evidence and LLM judgment: policy checks and trajectory replay establish that the work can be carried out correctly, while the provenance rubric assesses whether that work is recoverable from the agent-facing world. Once a sample is admitted, evaluated agents are scored using its database-level outcome and side-effect verifiers. Reliance on an LLM for the preceding provenance decision is an important limitation, which we discuss in the Limitations section.

\subsection{Evaluation Protocol}

Each benchmark task contains a natural-language instruction, an initial environment snapshot, an agent-facing workspace, and a verifier derived from the oracle transition. An agent succeeds when its final state contains the required changes, preserves the relevant policy invariants, and avoids unintended side effects. In infeasible cases, success requires identifying the blocker and stopping or refusing without corrupting the environment.

We use the control plane to define four complementary evaluation settings. In the \emph{Known-Workflow} setting, agents receive the relevant SOP and must execute it correctly under the current state and policies. In the \emph{Novel-Scenario} setting, agents must inspect records and retrieve the appropriate process documentation before deciding how to act. The \emph{Cross-Domain Orchestration} setting introduces dependencies across systems such as HR, ITSM, CSM, Drive, Email, and Calendar, as well as supporting actors whose information or approval is required. The \emph{Infeasibility Detection} setting evaluates whether agents can recognize impossible or unsafe requests and avoid harmful partial completion.

Together, these settings separate capabilities that are often conflated in enterprise-agent evaluation. Reliable agents must not only follow a known workflow; they must also find the relevant context, interpret organizational policy, coordinate with other actors, manage side effects across systems, and know when not to act.



==> ServiceNow/sections/methods_rough_sketch.tex <==
\section{Methods}

\ours{} is an environment-generation framework for constructing enterprise-agent benchmarks from executable software worlds. 
Most existing tool use benchmarks construct difficulty at the task level --- an expert or an LLM based pipeline authors a scenario, selects the records it touches, encodes the dependencies which make to hard and supplies a verifier. This approach often yields tasks with convoluted expected trajectory, or composed non-natural tasks. Our observations on production traces shows that most enterprises are deploying AI to follow their text based Standard Operating Procedures (workflows) to automate their daily tasks. Here the task complexity, often lies not in the nature of the task utterance, but the accumulated complexity of their enterprise world, where deployed agents have to operate under a confluence of edge cases of various sub-systems. 

Hence, we take a first principles approach to the problem to ask: how can we build benchmarks that reflect the true challenges encountered at deploy time. Difficulty should arise from the accumulated world state so that the same short, ordinary request can be easy, hard, or infeasible depending on the surrounding world context. We propose that if the forward simulation of "work" can be faithfully executed in the environment in a policy compliant way, benchmark task creation becomes a derivative of the simulation. The task utterance, and the final state verifiers (task completion, compliance, side effects etc) can be synthetically derived from the golden trajectory. We leverage information asymmetry as the guiding principle: during the construction time, the simulation agent operates in a over-specified world, where all organizational policies and workflows are encoded in code, and fail loudly when a write is policy violating. Later, during test time, we unwire all the tenant-specific organizational policies from the code wiring, and instead present them as a wiki of standard operating procedures and policies expressed in markdown format. Thus, during construction we can guarentee policy compliance, while at test time it becomes the responsibility of the agent reason through and follow the SOPs and policies, before committing any writes.

% Starting from a seeded enterprise state, the framework simulates business activity by running authored workflows through policy-gated tools. These executions produce valid state transitions from which we derive natural-language instructions, oracle trajectories, database-diff verifiers, and infeasible variants.

% The key design goal is to make task difficulty emerge from the environment rather than from prompt engineering. Instead of manually writing difficult scenarios and then constructing database states around them, \ours{} first builds causally rich enterprise snapshots through accumulated policy-valid activity. Executable workflows are then applied to these snapshots, so a short, ordinary request can be easy, difficult, or infeasible depending on the surrounding records, policies, approvals, and prior actions.


\subsection{Executable Enterprise Worlds}

We represent an enterprise environment as a tuple
\[
E = (O, D, P, T, K),
\]
where $O$ is the ontology, $D$ is the mutable database state, $P$ is the set of policies governing valid transitions, $T$ is the policy-gated tool surface, and $K$ is process knowledge. The ontology defines the relational schema of the enterprise world: tables, fields, foreign-key constraints, closed enum sets, and role or domain-specific entity types. The database stores the rows that instantiate this world at a given point in time. Policies encode both platform-level invariants (referential integrity, valid transitions etc) and tenant-configurable organizational rules (separation of duties, approval chains, compliance requirements) that determine which transactions are valid, and what rules apply. For example, a platform level policy could state that a new incident cannot move directly to closed state, where as an organizational policy states what process needs to be followed to make such transition (e.g. the VP needs to be informed when closing security related incidents). Tools are the only mechanism for changing the database: every write to $D$ passes through a tool and is checked against the relevant policies in $P$. Process knowledge consists of \textbf{executable workflows} during construction time, together with the policy and SOP documentation generated from them for the agent-facing workspace.

This representation makes consistency mechanical. Tools must reference real schema fields, workflows must call valid tools with valid arguments, policies must be satisfiable over the current database state, and generated states must satisfy the policy suite. As a result, \ours{} treats the enterprise environment as a runnable system with explicit invariants, rather than as a collection of manually authored tasks whose validity depends on review or LLM-as-judge evaluation.

\subsection{Generalizing Information Asymmetry}
The principle of Information asymmetry for benchmark construction leverages the controlled gap between the privileged vantage from which a task is built, and the partial vantage from which it must be solved. \cite{xie\section{Methods}

\ours{} is an environment-generation framework for constructing enterprise-agent benchmarks from executable software worlds. 
Most existing tool use benchmarks construct difficulty at the task level --- an expert or an LLM based pipeline authors a scenario, selects the records it touches, encodes the dependencies which make to hard and supplies a verifier. This approach often yields tasks with convoluted expected trajectory, or composed non-natural tasks. Our observations on production traces shows that most enterprises are deploying AI to follow their text based Standard Operating Procedures (workflows) to automate their daily tasks. Here the task complexity, often lies not in the nature of the task utterance, but the accumulated complexity of their enterprise world, where deployed agents have to operate under a confluence of edge cases of various sub-systems. 

Hence, we take a first principles approach to the problem to ask: how can we build benchmarks that reflect the true challenges encountered at deploy time. Difficulty should arise from the accumulated world state so that the same short, ordinary request can be easy, hard, or infeasible depending on the surrounding world context. We propose that if the forward simulation of "work" can be faithfully executed in the environment in a policy compliant way, benchmark task creation becomes a derivative of the simulation. The task utterance, and the final state verifiers (task completion, compliance, side effects etc) can be synthetically derived from the golden trajectory. We leverage information asymmetry as the guiding principle: during the construction time, the simulation agent operates in a over-specified world, where all organizational policies and workflows are encoded in code, and fail loudly when a write is policy violating. Later, during test time, we unwire all the tenant-specific organizational policies from the code wiring, and instead present them as a wiki of standard operating procedures and policies expressed in markdown format. Thus, during construction we can guarentee policy compliance, while at test time it becomes the responsibility of the agent reason through and follow the SOPs and policies, before committing any writes.

% Starting from a seeded enterprise state, the framework simulates business activity by running authored workflows through policy-gated tools. These executions produce valid state transitions from which we derive natural-language instructions, oracle trajectories, database-diff verifiers, and infeasible variants.

% The key design goal is to make task difficulty emerge from the environment rather than from prompt engineering. Instead of manually writing difficult scenarios and then constructing database states around them, \ours{} first builds causally rich enterprise snapshots through accumulated policy-valid activity. Executable workflows are then applied to these snapshots, so a short, ordinary request can be easy, difficult, or infeasible depending on the surrounding records, policies, approvals, and prior actions.


\subsection{Executable Enterprise Worlds}

We represent an enterprise environment as a tuple
\[
E = (O, D, P, T, K),
\]
where $O$ is the ontology, $D$ is the mutable database state, $P$ is the set of policies governing valid transitions, $T$ is the policy-gated tool surface, and $K$ is process knowledge. The ontology defines the relational schema of the enterprise world: tables, fields, foreign-key constraints, closed enum sets, and role or domain-specific entity types. The database stores the rows that instantiate this world at a given point in time. Policies encode both platform-level invariants (referential integrity, valid transitions etc) and tenant-configurable organizational rules (separation of duties, approval chains, compliance requirements) that determine which transactions are valid, and what rules apply. For example, a platform level policy could state that a new incident cannot move directly to closed state, where as an organizational policy states what process needs to be followed to make such transition (e.g. the VP needs to be informed when closing security related incidents). Tools are the only mechanism for changing the database: every write to $D$ passes through a tool and is checked against the relevant policies in $P$. Process knowledge consists of \textbf{executable workflows} during construction time, together with the policy and SOP documentation generated from them for the agent-facing workspace.

This representation makes consistency mechanical. Tools must reference real schema fields, workflows must call valid tools with valid arguments, policies must be satisfiable over the current database state, and generated states must satisfy the policy suite. As a result, \ours{} treats the enterprise environment as a runnable system with explicit invariants, rather than as a collection of manually authored tasks whose validity depends on review or LLM-as-judge evaluation.

\subsection{Generalizing Information Asymmetry}
The principle of Information asymmetry for benchmark construction leverages the controlled gap between the privileged vantage from which a task is built, and the partial vantage from which it must be solved. \cite{xie2026agentsynth} exploits this principle along a single axis --- that producing a solution trajectory by walking forward one tractable step at a time, is far easier than recovering the whole solution at once--- to make generation cheap and raise the difficulty with the length of the composed trajectory. The task and the verifiers are retro-derived from the trajectory. We generalize this principle along two further axes that are specifiec to constrained, policy governed work streams typical of Enterprises. 

\begin{itemize}
    \item \textbf{Trajectory} (\textit{shared with \cite{xie2026agentsynth}}) --- the oracle constructs the reference solution by executing the workflow forward; the agent however, must work out the trajectory from the workflow document.
    \item \textbf{Enforcement} --- during construction, the environment \textit{actively} enforces the organizational policy constraints and approvals. Failing policies can be backtracked and reattempted in a policy compliant way, and compliance approvals are readily obtained. During test, the tools no longer block policy violating actions, the agent is responsible for planning policy compliant actions, as well as communicating with other actors for approvals, information etc.
    \item \textbf{Specification} --- the policies and SOPs exist during construction as executable, machine checked artifacts, but exposed at test time ad prose documents the agent must read, interpret and map to the scenario at hand.
\end{itemize}

\subsection{World and Task Synthesis: Arrange, Act, Assert}
We prose to view the benchmark creation problem as a valid trajectory sampling problem. We can then use trajectories as the source of truth from which we generate the benchmark sample including the task document and the SQL  verifiers. The sample generation then reduces to three parts: 1) provisioning an initial world state 2) running a well-defined workflow and 3) deriving the task, environment edits and verifiers from the trajectory. 

Depending on the initial state provisioned, the workflow could branch in different ways, yielding diverse trajectories. Our proposed pipeline expects the the backend system and the formalized organizational knowledge as an input, and produces benchmark samples from it.  

\subsubsection{Backend System (Input)}
The backend system consists of the database schema, the organizational policies in python (read policies, and write policies) and MCP exposed tools which manipulate the backend state. These can be sourced either from live production systems, or authored by subject matter experts to mimic their enterprise's complexity and usage. The tools are wired to policies which block actions if the conditions are not satisfied. Furthermore, we expect organizational workflows implemented in python which capture the standard operating procedures of the organization. Each workflow is a decision tree, calling various policy wired tools or other workflows. \textcolor{red}{An illustration can be found in ... (TODO should make one diagram for this)}

\subsubsection{Arrange}
The first stage of the pipeline consists of provisioning a world to take actions on. This can be sourced from the real world when available. In this work, we create synthetic organizations spanning CSM, HR, ITSM and Medical domains with simulated db entities. Our world generation pipeline produces realistic, policy grounded enterprise operations databases from a declarative YAML archetype of the company, such as \texttt{saas\_midmarket}, \texttt{startup\_fast\_growth}, \texttt{regulated\_fintech} etc varying in scale of operations, domain ratios, customers etc. 
The scale and coverage of the seed world determines how many processes and their paths can execute in this world. We measure this by quantifying the \textit{yield} of the seed database state measured as the number of desirable paths of various workflows that can be executed in this world. To execute a given workflow on the world, we need to first bind the inputs of the workflow (for e.g. a HR onboarding workflow requires a new employee, the onboarding employee, and various other IDs in the HR system as inputs). Additionally, we are interested in covering the various edge cases that the workflow handles in our task, so as to drive the agent into trajectories where it would need to reason and handle these edge cases. Hence, we determine the \textit{interesting} paths in the workflow by doing a concolic walk over the python implementation of the workflow and endeavor to bind the entities which will drive the execution in that path. To this end, we built an agentic system to infer the pre-requisite conditions, i.e. what should be true in the world for a certain workflow to take a per-determined path? 

In Stage-1, we start with skeleton build with hierarchically organized and interconnected tables such as Organization, Groups \& Memberships, Customers, Profiles etc. Stage-2 enhances the skeleton by filling in realistic names, titles, descriptions, constraints etc. In stage-3, we simulate the operational state by driving real policy-gated tools to produce new incidents, problems, change requests, compliance records, notifications etc depending on the domain and the specific business logic. Finally we audit the generated DB to ensure coverage of various entities and their shapes, and database integrity and emit the final SQL statements to a portable SQL bundle to seed the world.db. This constitutes our seed world and allows for binding \textcolor{red}{70\%} of the paths directly. For the remaining \textcolor{red}{30\%}, we make surgical edits to the world state to allow for the binding of entities to match the concolic path. 

The output of the \textit{Arrange} stage includes the concolic paths, corresponding world db, and the input entity bindings. 

\subsubsection{Act}
In the \textit{Act}  stage, we sample a ground truth trajectory by running the workflow process on the bound entities for each path. For paths requiring approvals or other actions from other parties (such as VPs, manager, other department contacts, customers etc) a healer module automatically tracks requests for third party dependencies and auto-approves or auto-rejects based on the chosen concolic path and records them in the metadata. These third party actors are modeled as NPCs and simulated via LLMs conditioned on this metadata. The generated golden trajectory forms the basis for designing both the task prompt, as well as the SQL verifiers by inspecting the diff between the initial and final state. 
We also translate the python based process workflows into text based standard operating procedures Knowledge Base (SOP-KB) articles. Furthermore, we unwire the org policies  from the tools and expose the policies directly in the SOP-KBs. In this way, our proposal exploits information assymetry between sample construction time, and agent test time to generate hard, yet valid samples. During construction, the construction agent is assisted by the fact that tools fail loudly when violating policies, as well as the healer module supplying the golden NPC behavior. However, at test time, the agent needs to assess which tools are safe to call in a policy compliant way, and also figure out which NPC to interact with, as well as use the communication tools etc correctly to get to it's goal. Furthermore, the proposed approach allows for a control plane to test the agents in various scenarios such as re-wiring certain or all policies back with the tools, NPC behaviors, user providing additional context/clarification as needed etc. 

The output of the \textit{Act} stage includes the task document, corresponding SQL verifiers, and the rulebook for various NPCs and their behavior. 

\subsubsection{Assert}
Finally, we perform a rigorous quality check on the generated sample via LLM based rubrics. We perform this in two modes 1. on the golden trajectory itself and 2. contrastive comparison of a golden trajectory and a strong LLM agentic test time trajectory. 
For the golden trajectory, we check for provenance of each tool and parameter choice and if it's grounded in the given context such as the task document, SOP-KB articles and previous tool results. Additionally, we chose a strong LLM (Sonnet-5) with medium thinking in a ReAct orchestrator supplied with the oracle SOP-KB to check if it's trajectory either passes the verifier, or fails due to agent's mistake. Additionally, we also grade the samples on other qualitative metrics such as coherence, long horizon interestingness, etc. 

Finally, we include the best samples based on quality and rejection sampling for hardness. 

\subsection{Evaluation Protocol}

\ours{} evaluates agents on tasks drawn from evolved enterprise states. Each task includes a natural-language instruction, an initial environment snapshot, and a verifier derived from the oracle transition. An agent succeeds if its final environment state contains the required changes, preserves policy invariants, and avoids unintended side effects. In infeasible cases, the correct behavior is to identify the blocker and refuse or stop without corrupting state.

We organize evaluation into four complementary tracks. In the \textit{Known-Workflow} setting, agents receive the relevant process documentation (SOP-KB) and must execute it correctly under state and policy constraints. In the \textit{Novel-Scenario} setting, agents receive only the task and must inspect records, query related entities, infer missing constraints from tool feedback, and determine the correct procedure via retreiver based search. The \textit{Cross-Domain Orchestration} setting tests whether agents can coordinate actions across connected enterprise systems such as HR, ITSM, CSM, Drive, Email, and Calendar. The \textit{Infeasibility Detection} setting evaluates whether agents can recognize impossible or unsafe requests and avoid harmful partial completion.

Together, these tracks separate capabilities that are often conflated in enterprise-agent evaluation. Reliable agents must not only follow known workflows; they must also discover missing context, reason over stateful dependencies, coordinate across systems, and know when not to act.
2026agentsynth} exploits this principle along a single axis --- that producing a solution trajectory by walking forward one tractable step at a time, is far easier than recovering the whole solution at once--- to make generation cheap and raise the difficulty with the length of the composed trajectory. The task and the verifiers are retro-derived from the trajectory. We generalize this principle along two further axes that are specifiec to constrained, policy governed work streams typical of Enterprises. 

\begin{itemize}
    \item \textbf{Trajectory} (\textit{shared with \cite{xie2026agentsynth}}) --- the oracle constructs the reference solution by executing the workflow forward; the agent however, must work out the trajectory from the workflow document.
    \item \textbf{Enforcement} --- during construction, the environment \textit{actively} enforces the organizational policy constraints and approvals. Failing policies can be backtracked and reattempted in a policy compliant way, and compliance approvals are readily obtained. During test, the tools no longer block policy violating actions, the agent is responsible for planning policy compliant actions, as well as communicating with other actors for approvals, information etc.
    \item \textbf{Specification} --- the policies and SOPs exist during construction as executable, machine checked artifacts, but exposed at test time ad prose documents the agent must read, interpret and map to the scenario at hand.
\end{itemize}

\subsection{World and Task Synthesis: Arrange, Act, Assert}
We prose to view the benchmark creation problem as a valid trajectory sampling problem. We can then use trajectories as the source of truth from which we generate the benchmark sample including the task document and the SQL  verifiers. The sample generation then reduces to three parts: 1) provisioning an initial world state 2) running a well-defined workflow and 3) deriving the task, environment edits and verifiers from the trajectory. 

Depending on the initial state provisioned, the workflow could branch in different ways, yielding diverse trajectories. Our proposed pipeline expects the the backend system and the formalized organizational knowledge as an input, and produces benchmark samples from it.  

\subsubsection{Backend System (Input)}
The backend system consists of the database schema, the organizational policies in python (read policies, and write policies) and MCP exposed tools which manipulate the backend state. These can be sourced either from live production systems, or authored by subject matter experts to mimic their enterprise's complexity and usage. The tools are wired to policies which block actions if the conditions are not satisfied. Furthermore, we expect organizational workflows implemented in python which capture the standard operating procedures of the organization. Each workflow is a decision tree, calling various policy wired tools or other workflows. \textcolor{red}{An illustration can be found in ... (TODO should make one diagram for this)}

\subsubsection{Arrange}
The first stage of the pipeline consists of provisioning a world to take actions on. This can be sourced from the real world when available. In this work, we create synthetic organizations spanning CSM, HR, ITSM and Medical domains with simulated db entities. Our world generation pipeline produces realistic, policy grounded enterprise operations databases from a declarative YAML archetype of the company, such as \texttt{saas\_midmarket}, \texttt{startup\_fast\_growth}, \texttt{regulated\_fintech} etc varying in scale of operations, domain ratios, customers etc. 
The scale and coverage of the seed world determines how many processes and their paths can execute in this world. We measure this by quantifying the \textit{yield} of the seed database state measured as the number of desirable paths of various workflows that can be executed in this world. To execute a given workflow on the world, we need to first bind the inputs of the workflow (for e.g. a HR onboarding workflow requires a new employee, the onboarding employee, and various other IDs in the HR system as inputs). Additionally, we are interested in covering the various edge cases that the workflow handles in our task, so as to drive the agent into trajectories where it would need to reason and handle these edge cases. Hence, we determine the \textit{interesting} paths in the workflow by doing a concolic walk over the python implementation of the workflow and endeavor to bind the entities which will drive the execution in that path. To this end, we built an agentic system to infer the pre-requisite conditions, i.e. what should be true in the world for a certain workflow to take a per-determined path? 

In Stage-1, we start with skeleton build with hierarchically organized and interconnected tables such as Organization, Groups \& Memberships, Customers, Profiles etc. Stage-2 enhances the skeleton by filling in realistic names, titles, descriptions, constraints etc. In stage-3, we simulate the operational state by driving real policy-gated tools to produce new incidents, problems, change requests, compliance records, notifications etc depending on the domain and the specific business logic. Finally we audit the generated DB to ensure coverage of various entities and their shapes, and database integrity and emit the final SQL statements to a portable SQL bundle to seed the world.db. This constitutes our seed world and allows for binding \textcolor{red}{70\%} of the paths directly. For the remaining \textcolor{red}{30\%}, we make surgical edits to the world state to allow for the binding of entities to match the concolic path. 

The output of the \textit{Arrange} stage includes the concolic paths, corresponding world db, and the input entity bindings. 

\subsubsection{Act}
In the \textit{Act}  stage, we sample a ground truth trajectory by running the workflow process on the bound entities for each path. For paths requiring approvals or other actions from other parties (such as VPs, manager, other department contacts, customers etc) a healer module automatically tracks requests for third party dependencies and auto-approves or auto-rejects based on the chosen concolic path and records them in the metadata. These third party actors are modeled as NPCs and simulated via LLMs conditioned on this metadata. The generated golden trajectory forms the basis for designing both the task prompt, as well as the SQL verifiers by inspecting the diff between the initial and final state. 
We also translate the python based process workflows into text based standard operating procedures Knowledge Base (SOP-KB) articles. Furthermore, we unwire the org policies  from the tools and expose the policies directly in the SOP-KBs. In this way, our proposal exploits information assymetry between sample construction time, and agent test time to generate hard, yet valid samples. During construction, the construction agent is assisted by the fact that tools fail loudly when violating policies, as well as the healer module supplying the golden NPC behavior. However, at test time, the agent needs to assess which tools are safe to call in a policy compliant way, and also figure out which NPC to interact with, as well as use the communication tools etc correctly to get to it's goal. Furthermore, the proposed approach allows for a control plane to test the agents in various scenarios such as re-wiring certain or all policies back with the tools, NPC behaviors, user providing additional context/clarification as needed etc. 

The output of the \textit{Act} stage includes the task document, corresponding SQL verifiers, and the rulebook for various NPCs and their behavior. 

\subsubsection{Assert}
Finally, we perform a rigorous quality check on the generated sample via LLM based rubrics. We perform this in two modes 1. on the golden trajectory itself and 2. contrastive comparison of a golden trajectory and a strong LLM agentic test time trajectory. 
For the golden trajectory, we check for provenance of each tool and parameter choice and if it's grounded in the given context such as the task document, SOP-KB articles and previous tool results. Additionally, we chose a strong LLM (Sonnet-5) with medium thinking in a ReAct orchestrator supplied with the oracle SOP-KB to check if it's trajectory either passes the verifier, or fails due to agent's mistake. Additionally, we also grade the samples on other qualitative metrics such as coherence, long horizon interestingness, etc. 

Finally, we include the best samples based on quality and rejection sampling for hardness. 

\subsection{Evaluation Protocol}

\ours{} evaluates agents on tasks drawn from evolved enterprise states. Each task includes a natural-language instruction, an initial environment snapshot, and a verifier derived from the oracle transition. An agent succeeds if its final environment state contains the required changes, preserves policy invariants, and avoids unintended side effects. In infeasible cases, the correct behavior is to identify the blocker and refuse or stop without corrupting state.

We organize evaluation into four complementary tracks. In the \textit{Known-Workflow} setting, agents receive the relevant process documentation (SOP-KB) and must execute it correctly under state and policy constraints. In the \textit{Novel-Scenario} setting, agents receive only the task and must inspect records, query related entities, infer missing constraints from tool feedback, and determine the correct procedure via retreiver based search. The \textit{Cross-Domain Orchestration} setting tests whether agents can coordinate actions across connected enterprise systems such as HR, ITSM, CSM, Drive, Email, and Calendar. The \textit{Infeasibility Detection} setting evaluates whether agents can recognize impossible or unsafe requests and avoid harmful partial completion.

Together, these tracks separate capabilities that are often conflated in enterprise-agent evaluation. Reliable agents must not only follow known workflows; they must also discover missing context, reason over stateful dependencies, coordinate across systems, and know when not to act.


==> ServiceNow/sections/related_works.tex <==
\section{Related Works}


\paragraph{Agent and tool-use benchmarks.}
Existing benchmarks evaluate LLM agents through APIs, tools, browsers, desktops, terminals, and other executable environments. Tool-use benchmarks emphasize tool selection, argument grounding, and multi-step invocation~\citep{li2023apibank,qin2024toolllm,chen2025acebench,yao2025taubench,barres2025tau2}; web and computer-use benchmarks study long-horizon interaction through graphical interfaces and operating systems~\citep{yao2022webshop,zhou2023webarena,xie2024osworld,bonatti2024windowsagentarena,nayak2025uivision}; and software-engineering and terminal benchmarks require agents to inspect system state, modify artifacts, and execute extended workflows~\citep{jimenez2024swebench,merrill2026terminal,yang2026programbenchlanguagemodelsrebuild}. These benchmarks primarily measure execution within a predefined task and environment. We instead study how the surrounding world---its prior state, policies, linked records, and dependencies---can make the same simple request easy, difficult, or infeasible.

% \paragraph{Agent and tool-use benchmarks.}
% A growing body of work evaluates LLM agents that act through tools, APIs, browsers, desktops, and executable software environments. General tool-use benchmarks study API invocation, tool selection, argument grounding, and multi-step tool chaining~\citep{li2023apibank,qin2024toolllm,chen2025acebench,yao2025taubench,barres2025tau2}, while web and computer-use benchmarks evaluate long-horizon interaction through graphical interfaces and operating systems~\citep{yao2022webshop, zhou2023webarena,xie2024osworld,bonatti2024windowsagentarena,nayak2025uivision}. Software-engineering and terminal benchmarks instead place agents in executable environments, where they must inspect repositories or system state, modify artifacts, invoke commands and tests, and complete extended workflows~\citep{jimenez2024swebench,merrill2026terminal}. ProgramBench pushes this direction toward holistic software construction by asking agents to recreate complete programs from documentation and the behavior of a reference executable~\citep{yang2026programbenchlanguagemodelsrebuild}. 
% Collectively, these benchmarks measure whether agents can plan, choose actions, use tools correctly, recover from errors, and complete realistic software tasks. Their difficulty, however, remains largely \emph{intrinsic to a predefined task and environment}: each agent is placed in a fixed setting and judged on how well it executes within it. They less directly probe the regime we target, where an otherwise simple request is made easy, difficult, or infeasible by the surrounding world, including its prior state, linked records, organizational policies, and cross-record dependencies.


\paragraph{Professional and enterprise agents.}
Professional benchmarks evaluate economically meaningful deliverables or workplace activity, including expert-authored occupational tasks in GDPval and simulated organizational work in TheAgentCompany~\citep{patwardhan2025gdpval,xu2026theagentcompany}. Enterprise benchmarks further ground agents in business applications, mutable operational data, and organizational procedures. WorkArena and WorkArena++ evaluate ServiceNow workflows; CRMArena and CRMArena-Pro cover Salesforce processes; SOP-Bench studies industrial procedures; and AutomationBench introduces cross-application workflows with business rules and programmatic verification~\citep{drouin2024workarena,boisvert2024workarenaplusplus,huang2025crmarena,huang2025crmarena_pro,nandi2025sopbench,shepard2026automationbench}. EntCollabBench additionally studies delegation and approval decisions among permission-isolated agents~\citep{yu2026beyond}. EnterpriseOps-Gym is the closest precursor, combining multi-domain tools, persistent relational state, policy constraints, infeasible tasks, and database-level verification~\citep{malay2026enterpriseopsgym}. \ours{} changes the unit of construction: rather than authoring tasks against configured snapshots, it evolves a shared enterprise through policy-valid activity and derives tasks, oracle trajectories, and verifiers from the resulting transitions. Enterprise state is therefore not merely task context, but the substrate from which tasks are generated.

% \paragraph{Professional and enterprise agents.}
% A complementary line of work asks whether agents can perform economically meaningful work rather than isolated tool-use tasks. GDPval evaluates expert-authored deliverables across a broad range of occupations, while TheAgentCompany places agents in a simulated software company where they interact with internal websites, execute code, and communicate with coworkers~\citep{patwardhan2025gdpval,xu2026theagentcompany}. These benchmarks broaden evaluation toward realistic professional outcomes and workplace activity, but their primary focus is the fidelity and economic relevance of the work being performed. Interactive enterprise benchmarks instead ground agents in business applications, organizational procedures, and mutable operational data. WorkArena and WorkArena++ instantiate knowledge-work workflows in ServiceNow, while CRMArena and CRMArena-Pro evaluate agents on realistic Salesforce CRM processes and interactions~\citep{drouin2024workarena,boisvert2024workarenaplusplus,huang2025crmarena,huang2025crmarena_pro}. SOP-Bench focuses on executing complex industrial procedures, whereas AutomationBench evaluates cross-application API workflows under layered business rules, irrelevant or misleading records, and programmatic end-state verification~\citep{nandi2025sopbench,shepard2026automationbench}. Recent work further incorporates organizational structure: EntCollabBench studies collaboration among permission-isolated, role-specialized agents, including delegation and policy-grounded approval decisions~\citep{yu2026beyond}. EnterpriseOps-Gym is the closest precursor to our setting, combining multi-domain tools with persistent relational state, policy constraints, infeasible tasks, and database-level verification~\citep{malay2026enterpriseopsgym}. \ours{} builds on this progression but changes the unit of benchmark construction: rather than authoring a task and configuring a compatible snapshot, it evolves a shared enterprise through policy-valid activity and derives tasks from the resulting verified transitions. Each task therefore inherits its preconditions, governing policies, oracle trajectory, and expected state change from the history that produced it. In \ours{}, enterprise state is not merely part of task setup; it is the substrate from which tasks and their verifiers are generated.

\paragraph{Scaling and evolving agent environments.}
Recent work synthesizes executable environments and verifiable tasks at scale. Endless Terminals generates containerized terminal tasks and tests; Gym-Anything and CUA-Gym construct interactive applications together with realistic states, tasks, and reward functions~\citep{gandhi2026endless,aggarwal2026gymanythingturnsoftwareagent,wang2026cua}. EnvScaler and EnvFactory synthesize stateful tool environments and grounded trajectories, ComplexMCP targets large interdependent tool ecosystems, and TASTE derives tasks from explored tool sequences~\citep{song2026envscaler,xu2026envfactoryscalingtooluseagents,li2026complexmcp,keren2026mattertasteimprovingcoverage}. ProEvolve instead transforms an environment graph of schemas, data, and tools to create successive environment versions~\citep{li2026proevolve}. \ours{} studies a complementary form of evolution: the endogenous state of one persistent, policy-governed enterprise changes through simulated business activity. Tasks derived from this history can depend on earlier events, become infeasible through state-dependent blockers, and be verified against both database effects and policy invariants.
% maybe cite chen2025learning, title={Learning evolving tools for large language models},

% \paragraph{Scaling and evolving agent environments.}
% A rapidly growing line of work treats executable environments and verifiable tasks as objects that can themselves be synthesized at scale. Endless Terminals procedurally generates terminal tasks together with containerized environments and completion tests, while Gym-Anything converts arbitrary software into interactive computer-use environments populated with realistic data and long-horizon tasks~\citep{gandhi2026endless,aggarwal2026gymanythingturnsoftwareagent}. CUA-Gym similarly co-generates task instructions, initial and target application states, and executable reward functions across a large collection of mock applications~\citep{wang2026cua}. For tool-using agents, EnvScaler and EnvFactory automate the construction of stateful tool environments and the synthesis of grounded scenarios or trajectories within them~\citep{song2026envscaler,xu2026envfactoryscalingtooluseagents}; ComplexMCP instead emphasizes large, interdependent, and stochastic tool ecosystems~\citep{li2026complexmcp}, while TASTE reverses conventional task authoring by first exploring the space of valid tool sequences and then instantiating tasks around selected sequences~\citep{keren2026mattertasteimprovingcoverage}. Closest in motivation, ProEvolve explicitly represents schemas, data, and tools as an environment graph and applies coordinated transformations to produce successive environment versions~\citep{li2026proevolve}. \ours{} shares the goal of moving beyond manual, task-by-task authoring, but studies a complementary form of evolution. Rather than primarily scaling across independently generated environments, task instances, or structural versions of an environment, \ours{} evolves the \emph{endogenous state} of a persistent, policy-governed enterprise through simulated business activity. Tasks are then derived from the verified transitions in this evolving history. Consequently, task difficulty can depend on events that occurred long before the task was issued, infeasibility can emerge naturally from state-dependent blockers, and outcomes can be verified against both expected database changes and policy invariants.

\paragraph{Privileged information in task generation.}
Several approaches exploit information available during task construction but hidden during evaluation. This resembles learning using privileged information~\citep{vapnik2009lupi}, but moves the asymmetry from model training to benchmark generation. AgentSynth uses construction-time subtasks and trajectories to compose harder tasks, while Endless Terminals uses hidden ground-truth descriptions for generation and verification~\citep{xie2026agentsynth,gandhi2026endless}. In \ours{}, the privileged object is an executable policy representation: during construction, it validates every world transition; during evaluation, it is withheld, requiring the agent to recover the applicable rules from ordinary workspace documentation.

% \paragraph{Privileged information in task generation.}
% A separate thread exploits an asymmetry between what is available when a task is \emph{constructed} and what is exposed to the agent that is later \emph{evaluated} on it. This mirrors the classical learning using privileged information (LUPI) setting, where side information available at training time is withheld at test time~\citep{vapnik2009lupi}, but moves the asymmetry upstream from model training to task and environment generation. AgentSynth uses the intermediate subtasks and trajectories available during forward construction to synthesize harder composite tasks, while Endless Terminals relies on privileged ground-truth descriptions to construct and verify tasks without revealing them to the evaluated agent~\citep{xie2026agentsynth,gandhi2026endless}. \ours{} instantiates this principle with a specific privileged object: an executable representation of organizational policy that governs how the enterprise world may evolve. During construction, this policy oracle enforces the validity of every transition; at evaluation, it is withheld, and the agent must recover the same rules from ordinary workspace knowledge before acting.

==> ServiceNow/sections/related_works_old.tex <==
\section{Related Works}


\paragraph{Agent and tool-use benchmarks.}
A growing body of work evaluates LLM agents that act through tools, APIs, browsers, desktops, and executable software environments. General tool-use benchmarks study API invocation, tool selection, argument grounding, and multi-step tool chaining~\citep{li2023apibank,qin2024toolllm,chen2025acebench,yao2025taubench,barres2025tau2}, while web and computer-use benchmarks evaluate long-horizon interaction through graphical interfaces and operating systems~\citep{yao2022webshop, zhou2023webarena,xie2024osworld,bonatti2024windowsagentarena,nayak2025uivision}. Software-engineering and terminal benchmarks instead place agents in executable environments, where they must inspect repositories or system state, modify artifacts, invoke commands and tests, and complete extended workflows~\citep{jimenez2024swebench,merrill2026terminal}. ProgramBench pushes this direction toward holistic software construction by asking agents to recreate complete programs from documentation and the behavior of a reference executable~\citep{yang2026programbenchlanguagemodelsrebuild}. 
Collectively, these benchmarks measure whether agents can plan, choose actions, use tools correctly, recover from errors, and complete realistic software tasks. Their difficulty, however, remains largely \emph{intrinsic to a predefined task and environment}: each agent is placed in a fixed setting and judged on how well it executes within it. They less directly probe the regime we target, where an otherwise simple request is made easy, difficult, or infeasible by the surrounding world, including its prior state, linked records, organizational policies, and cross-record dependencies.



\paragraph{Professional and enterprise agents.}
A complementary line of work asks whether agents can perform economically meaningful work rather than isolated tool-use tasks. GDPval evaluates expert-authored deliverables across a broad range of occupations, while TheAgentCompany places agents in a simulated software company where they interact with internal websites, execute code, and communicate with coworkers~\citep{patwardhan2025gdpval,xu2026theagentcompany}. These benchmarks broaden evaluation toward realistic professional outcomes and workplace activity, but their primary focus is the fidelity and economic relevance of the work being performed. Interactive enterprise benchmarks instead ground agents in business applications, organizational procedures, and mutable operational data. WorkArena and WorkArena++ instantiate knowledge-work workflows in ServiceNow, while CRMArena and CRMArena-Pro evaluate agents on realistic Salesforce CRM processes and interactions~\citep{drouin2024workarena,boisvert2024workarenaplusplus,huang2025crmarena,huang2025crmarena_pro}. SOP-Bench focuses on executing complex industrial procedures, whereas AutomationBench evaluates cross-application API workflows under layered business rules, irrelevant or misleading records, and programmatic end-state verification~\citep{nandi2025sopbench,shepard2026automationbench}. Recent work further incorporates organizational structure: EntCollabBench studies collaboration among permission-isolated, role-specialized agents, including delegation and policy-grounded approval decisions~\citep{yu2026beyond}. EnterpriseOps-Gym is the closest precursor to our setting, combining multi-domain tools with persistent relational state, policy constraints, infeasible tasks, and database-level verification~\citep{malay2026enterpriseopsgym}. \ours{} builds on this progression but changes the unit of benchmark construction: rather than authoring a task and configuring a compatible snapshot, it evolves a shared enterprise through policy-valid activity and derives tasks from the resulting verified transitions. Each task therefore inherits its preconditions, governing policies, oracle trajectory, and expected state change from the history that produced it. In \ours{}, enterprise state is not merely part of task setup; it is the substrate from which tasks and their verifiers are generated.


\paragraph{Scaling and evolving agent environments.}
A rapidly growing line of work treats executable environments and verifiable tasks as objects that can themselves be synthesized at scale. Endless Terminals procedurally generates terminal tasks together with containerized environments and completion tests, while Gym-Anything converts arbitrary software into interactive computer-use environments populated with realistic data and long-horizon tasks~\citep{gandhi2026endless,aggarwal2026gymanythingturnsoftwareagent}. CUA-Gym similarly co-generates task instructions, initial and target application states, and executable reward functions across a large collection of mock applications~\citep{wang2026cua}. For tool-using agents, EnvScaler and EnvFactory automate the construction of stateful tool environments and the synthesis of grounded scenarios or trajectories within them~\citep{song2026envscaler,xu2026envfactoryscalingtooluseagents}; ComplexMCP instead emphasizes large, interdependent, and stochastic tool ecosystems~\citep{li2026complexmcp}, while TASTE reverses conventional task authoring by first exploring the space of valid tool sequences and then instantiating tasks around selected sequences~\citep{keren2026mattertasteimprovingcoverage}. Closest in motivation, ProEvolve explicitly represents schemas, data, and tools as an environment graph and applies coordinated transformations to produce successive environment versions~\citep{li2026proevolve}. \ours{} shares the goal of moving beyond manual, task-by-task authoring, but studies a complementary form of evolution. Rather than primarily scaling across independently generated environments, task instances, or structural versions of an environment, \ours{} evolves the \emph{endogenous state} of a persistent, policy-governed enterprise through simulated business activity. Tasks are then derived from the verified transitions in this evolving history. Consequently, task difficulty can depend on events that occurred long before the task was issued, infeasibility can emerge naturally from state-dependent blockers, and outcomes can be verified against both expected database changes and policy invariants.

\paragraph{Privileged information in task generation.}
A separate thread exploits an asymmetry between what is available when a task is \emph{constructed} and what is exposed to the agent that is later \emph{evaluated} on it. This mirrors the classical learning using privileged information (LUPI) setting, where side information available at training time is withheld at test time~\citep{vapnik2009lupi}, but moves the asymmetry upstream from model training to task and environment generation. AgentSynth uses the intermediate subtasks and trajectories available during forward construction to synthesize harder composite tasks, while Endless Terminals relies on privileged ground-truth descriptions to construct and verify tasks without revealing them to the evaluated agent~\citep{xie2026agentsynth,gandhi2026endless}. \ours{} instantiates this principle with a specific privileged object: an executable representation of organizational policy that governs how the enterprise world may evolve. During construction, this policy oracle enforces the validity of every transition; at evaluation, it is withheld, and the agent must recover the same rules from ordinary workspace knowledge before acting.

==> ServiceNow/sections/results.tex <==
\section{Experiments and Results}

\begin{table}[ht]
\caption{\textcolor{red}{PLACEHOLDER TABLE FOR RESULTS}}
\label{tab:results}
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Dataset} & \textbf{Naive} & \textbf{Flexible} & \textbf{Better?} \\
\midrule
Breast  & $95.9 \pm 0.2$ & $96.7 \pm 0.2$ & \(\checkmark\) \\
Cleve   & $81.3 \pm 0.6$ & $80.0 \pm 0.6$ & \(\checkmark\) \\
Glass2  & $61.9 \pm 1.4$ & $83.8 \pm 0.7$ &  \\
Credit  & $74.8 \pm 0.5$ & $78.3 \pm 0.6$ & \(\checkmark\) \\
Horse   & $73.3 \pm 0.9$ & $69.7 \pm 1.0$ & \(\checkmark\) \\
Meta    & $67.1 \pm 0.6$ & $76.5 \pm 0.5$ & \(\checkmark\) \\
Pima    & $75.1 \pm 0.6$ & $73.9 \pm 0.5$ &  \\
Vehicle & $44.9 \pm 0.6$ & $61.5 \pm 0.4$ & \(\checkmark\) \\
\bottomrule
\end{tabular}
\end{table}


==> ServiceNow/team_related_work/ui_assist.tex <==
% BrowserGym ecosystem
The BrowserGym Ecosystem for Web Agent Research paper \citep{dechezelles2025browsergymecosystemwebagent} introduces a standardized, gym-like framework that unifies diverse web agent benchmarks and integrates tools like AgentLab to enable consistent evaluation, development, and analysis of LLM-driven web agents. Using this ecosystem, the authors run large-scale experiments across multiple benchmarks to compare state-of-the-art models, highlighting significant performance differences and ongoing challenges in building robust web agents.

% WorkArena and WorkArena ++
WorkArena \citep{drouin2024workarena} troduces a benchmark of realistic enterprise browser tasks and uses the BrowserGym environment to evaluate how well LLM-driven web agents handle common knowledge work activities, revealing a substantial gap between current agent performance and full task automation. WorkArena++ \citep{boisvert2024workarena++} significantly expands on this by offering hundreds of compositional, multi-step enterprise tasks designed to test planning, reasoning, and complex problem-solving skills of web agents, showing that today’s models still struggle compared to humans.  

% How To train your LLM Web Agent
How to Train Your LLM Web Agent: A Statistical Diagnosis \citep{vattikonda2025train} presents a statistically grounded, compute-Pareto-optimal training pipeline that combines supervised fine-tuning from a large teacher with on-policy reinforcement learning for a smaller student, achieving superior performance–compute trade-offs compared to SFT-only or RL-only baselines. The work includes a detailed statistical analysis of optimal hyperparameters and their sensitivity to the initial SFT warm-up phase, and demonstrates consistent gains on multi-step benchmarks such as WorkArena and MiniWob++ while substantially reducing total training compute.

% Jeff-Hinter
Just-in-time Episodic Feedback Hinter (JEF-Hinter) \citep{nekoei2025just} introduces a lightweight agentic system that distills offline trajectories into compact, context-aware hints via a “zoom \& reflect” pipeline, guiding LLM agents at inference time without fine-tuning and outperforming strong baselines on MiniWoB++, WorkArena-L1, and WebArena-Lite. By leveraging both successful and failed traces and enabling parallel hint generation and retrieval, JEF-Hinter improves adaptation and robustness in sequential decision tasks with minimal extra compute and transparent, traceable feedback integration. 
